Differentially Private Decoupled Graph Convolutions for Multigranular Topology Protection

GNNs can inadvertently expose sensitive user information and interactions through their model predictions. To address these privacy concerns, Differential Privacy (DP) protocols are employed to control the trade-off between provable privacy protection and model utility. Applying standard DP approaches to GNNs directly is not advisable due to two main reasons. First, the prediction of node labels, which relies on neighboring node attributes through graph convolutions, can lead to privacy leakage. Second, in practical applications, the privacy requirements for node attributes and graph topology may differ. In the latter setting, existing DP-GNN models fail to provide multigranular trade-offs between graph topology privacy, node attribute privacy, and GNN utility. To address both limitations, we propose a new framework termed Graph Differential Privacy (GDP), specifically tailored to graph learning. GDP ensures both provably private model parameters as well as private predictions. Additionally, we describe a novel unified notion of graph dataset adjacency to analyze the properties of GDP for different levels of graph topology privacy. Our findings reveal that DP-GNNs, which rely on graph convolutions, not only fail to meet the requirements for multigranular graph topology privacy but also necessitate the injection of DP noise that scales at least linearly with the maximum node degree. In contrast, our proposed Differentially Private Decoupled Graph Convolutions (DPDGCs) represent a more flexible and efficient alternative to graph convolutions that still provides the necessary guarantees of GDP. To validate our approach, we conducted extensive experiments on seven node classification benchmarking and illustrative synthetic datasets. The results demonstrate that DPDGCs significantly outperform existing DP-GNNs in terms of privacy-utility trade-offs.

==> macro_wnchen.tex <==
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left[}
\newcommand{\rb}{\right]}
\newcommand{\lbp}{\left\{}
\newcommand{\rbp}{\right\}}
\newcommand{\lba}{\left\lvert}
\newcommand{\rba}{\right\rvert}
\newcommand{\lV}{\left\lVert}
\newcommand{\rV}{\right\rVert}
\newcommand{\mv}{\middle\vert}
\newcommand{\ul}{\underline}
\newcommand{\ol}{\overline}
\newcommand{\mcal}{\mathcal}
\newcommand{\mscr}{\mathscr}
\newcommand{\what}{\widehat}
\newcommand{\wtild}{\widetilde}
\newcommand{\mb}{\mathbf}
\newcommand{\bbm}{\mathbbm}
\newcommand{\mbb}{\mathbb}
\newcommand{\msf}{\mathsf}
\newcommand{\la}{\leftarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\ua}{\uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\lgla}{\longleftarrow}
\newcommand{\lgra}{\longrightarrow}
\newcommand{\lglra}{\longleftrightarrow}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\llan}{\left\langle}
\newcommand{\rran}{\right\rangle}
\newcommand{\lce}{\left\lceil}
\newcommand{\rce}{\right\rceil}
\newcommand{\lfl}{\left\lfloor}
\newcommand{\rfl}{\right\rfloor}

==> sec_dpgnn_alg.tex <==
\section{Practical Privacy Accounting}
Below, we describe the detailed steps of DP-GNN in Algorithm~\ref{alg:dpgnn}. Notice that we will account for the privacy budget with R\'enyi DP \cite{mironov2017renyi} across $T$ training epochs (which allows tighter privacy constants compared to classical advanced composition theorem \cite{kairouz2015composition}), but we can convert the final R\'enyi DP guarantee to standard $\left(\varepsilon_{\mathsf{DP}}(\delta), \delta\right)$-DP through the following conversion lemma from \cite{asoodeh2020better, canonne2020discrete, bun2016concentrated}:
\begin{lemma}\label{lemma:rdp_to_approx_dp}
    If a randomized mechanism $\mathcal{M}$ satisfies $\left( \alpha, \varepsilon(\alpha) \right)$-RDP for all $\alpha > 1$, then, for any $\delta > 0$, $M$ satisfies $\left( \varepsilon_{\mathsf{DP}}(\delta), \delta \right)$-DP, where
$$ \varepsilon_{\mathsf{DP}}(\delta) = \inf_{\alpha > 1}\varepsilon(\alpha)+\frac{\log\left( 1/\alpha\delta \right)}{\alpha-1}+\log(1-1/\alpha). $$
\end{lemma}

We summarize the proposed DP-GNN in Algorithm~\ref{alg:dpgnn}, and the resulting DP guarantees are given in the following theorem.

\begin{theorem}
Algorithm~\ref{alg:dpgnn} satisfies $(\varepsilon(\alpha), \alpha)$-R\'enyi DP for all
$$ \varepsilon(\alpha) \geq  T\alpha\left( \frac{L^2_\mathbf{w}}{2\sigma^2_\mathbf{w}} +  \frac{L^2_\mathbf{\gamma}}{2\sigma^2_\mathbf{\gamma}}\right), $$
where $L_\mathbf{w}$ and $L_\mathbf{\gamma}$ are the $\ell_2$ sensitivity bound given in \eqref{} and \eqref{}. In addition, if $\varepsilon = O(1)$, then setting
$$ \sigma^2_\mathbf{w} = O\left( \frac{L_\mathbf{w}\sqrt{T\log(1/\delta)}}{\varepsilon} \right) \, \text{ and } \sigma^2_\mathbf{\gamma} = O\left( \frac{L_\mathbf{\gamma}\sqrt{T\log(1/\delta)}}{\varepsilon} \right)$$
yields $(\varepsilon, \delta)$-(approximate) DP.
\end{theorem}


\begin{algorithm}[h]
\caption{Differentially Private Graph Neural Networks}\label{alg:dpgnn}
\begin{algorithmic}
    \STATE {\bfseries Input:} Node features $\bm{X} \in \mathbb{R}^{n \times F}$, Graph $\mathcal{G} = \left( \mathcal{V}, \mathcal{E} \right)$, Privacy budgets $(\varepsilon, \delta)$.
    \STATE Initialize $\mathbf{w}_0$ and $\mathbf{\gamma}^{(0)} = \left( \frac{1}{K}, ..., \frac{1}{K} \right)$
    \FOR{epoch $t = 1,..., T$}
	\STATE Compute the (clipped) gradients 
 $ D_{\mathbf{w}}L(\mathbf{\Theta};\mathcal{D})$ and $ D_{\mathbf{\gamma}}L\left( \mathbf{\Theta}; \mathcal{D} \right)$
 \STATE Update the model: $$\mathbf{w}_t \leftarrow D_{\mathbf{w}}L\left( \Theta; \mathcal{D} \right) + N\left( 0, \sigma_\mathbf{w}^2 \right), \, \text{ and } \mathbf{\gamma}_t \leftarrow D_{\mathbf{\gamma}}L\left( \Theta; \mathcal{D} \right) + N\left( 0, \sigma_\mathbf{\gamma}^2 \right),$$ where $\sigma_\mathbf{w}^2$ and $\sigma_\mathbf{\gamma}^2$ are computed according to Algorithm~\ref{alg:dp_budgetting}.
    \ENDFOR
	\STATE {\bfseries Return:} $(\mathbf{w}_T, \mathbf{\gamma}_T)$
\end{algorithmic}
\end{algorithm}

In practice, when we are given a $(\varepsilon, \delta)$ privacy budget and a \emph{splitting ratio} $\eta$ that specifies the ratio of budgets for privatizing $ D_{\mathbf{w}}L(\mathbf{\Theta};\mathcal{D})$ and $D_{\mathbf{\gamma}}L\left( \mathbf{\Theta}; \mathcal{D} \right)$, we perform Algorithm~\ref{alg:dp_budgetting} to determine $(\sigma_\mathbf{w}, \sigma_\mathbf{\gamma})$.


\begin{algorithm}[h]
\caption{Privacy Budgetting}\label{alg:dp_budgetting}
\begin{algorithmic}
    \STATE {\bfseries Input:} $\ell_2$ sensitivity $L_\mathbf{w}$ and $L_\mathbf{\gamma}$, privacy budget $(\varepsilon, \delta)$, splitting ratio $\eta \in (0, 1)$, number of rounds $T$.
    \STATE Find smallest noise multiplier $\nu > 0$ such that the following inequality holds:
    $$ \varepsilon \geq \inf_{\alpha > 1}\frac{\alpha}{2\nu^2}+\frac{\log\left( 1/\alpha\delta \right)}{\alpha-1}+\log(1-1/\alpha).$$
    Set $\sigma_\mathbf{w} = \frac{1}{\eta}L_\mathbf{w}\cdot\nu$ and  $\sigma_\mathbf{\gamma} = \left(\frac{1}{\eta}-1\right)L_\mathbf{\gamma}\cdot \nu$
	\STATE {\bfseries Return:} Noise magnitudes $(\sigma_\mathbf{w}, \sigma_\mathbf{\gamma})$.
\end{algorithmic}
\end{algorithm}

